On the variance of radio interferometric calibration solutions: Quality-based Weighting Schemes

This paper investigates the possibility of improving radio interferometric images using an algorithm inspired by an optical method known as "lucky imaging", which would give more weight to the best-calibrated visibilities used to make a given image. A fundamental relationship between the statistics of interferometric calibration solution residuals and those of the image-plane pixels is derived in this paper. This relationship allows us to understand and describe the statistical properties of the residual image. In this framework, the noise-map can be described as the Fourier transform of the covariance between residual visibilities in a new differential Fourier plane. Image-plane artefacts can be seen as one realisation of the pixel covariance distribution, which can be estimated from the antenna gain statistics. Based on this relationship, we propose a means of improving images made with calibrated visibilities using weighting schemes. This improvement would occur after calibration, but before imaging - it is thus ideally used between major iterations of self-calibration loops. Applying the weighting scheme to simulated data improves the noise level in the final image at negligible computational cost.

==> source/copy_of_matrix-algorithm.tex <==
\section{Estimating the Covariance Matrix}\label{section.algorithm}
\pg
In our simulations, we have worked from a known covariance matrix and shown that our predictions for the residual image's behaviour hold. With real data, however, we do not have access to this underlying covariance matrix for each baseline. Since our weights are extracted from the covariance matrices, a significant obstacle to overcome is to estimate them as accurately as possible.


\pg
To begin, we will retrace the steps of Section \ref{sec.formalism}. In the absence of direction-dependent effects, we define the residual matrix as:
\begin{align}
\Rmat{\tnuIndeix} =& \sum_d s_d \Kmat{d,\tnuIndeix} ( \VarmatTau ) \Kmat{d,\tnuIndeix}^H + n \label{eq.residual.matrix}
\end{align}
where we assume that we do not have direction-dependent gains: $\VarmatTau$ is then the same for all directions. The K-matrix is defined as follows:
\begin{align}
%\Kmat{d} =&
%\begin{pmatrix}
%k_{p,\tnuIndeix}^{d}   &         &                       &   0     &\\
%                       &  \ddots &                       &        &\\
%                       &         & k_{q,\tnuIndeix'}^{d} &        &\\ 
%          0             &         &                       & \ddots 
%\end{pmatrix}
%\quad
\Kmat{d,\tnuIndeix} =&
\begin{pmatrix}
k_{p,\tnuIndeix}^{d}   &                       &   0     &\\
                       & k_{q,\tnuIndeix}^{d}  &        &\\ 
         0              &                       & \ddots 
\end{pmatrix}
\end{align}



\pg
Since the residual matrix depends on the gains, we define the residual visibility vectors as:
\begin{align}
\Rmat{{\cellindex}} =&   \begin{pmatrix} \vdots \\ \Rmat{\tnuIndeix\in \cellindex} \\ \vdots \end{pmatrix} \\
\Rmat{} =&   \begin{pmatrix} \hdots \quad \Rmat{c} \quad \hdots \end{pmatrix}
\end{align}

\pg
$\Rmat{\cellindex}$ corresponds to a matrix containing all the residual visibilities within one calibration cell $\cellindex$, i.e. for $\tnuIndeix \in \cellindex$ where $\gvect_{\cellindex} = \const$ The residual variance sample matrix can now be built by multiplying the residual visibility vector with its Hermitian conjugate:
\begin{align}
\matVV             =& \Rmat{}^H \Rmat{} \label{eq.matvv.definition} %\\
%                   =& (\sum_d s_d \Kmat{d} \Varmat \Kmat{d}^H)^H(\sum_d s_d \Kmat{d} ( \Varmat ) \Kmat{d}^H)\\
%                   =& (\sum_d s_d \Kmat{d}^H \Varmat^H \Kmat{d})(\sum_d s_d \Kmat{d} ( \Varmat ) \Kmat{d}^H)\\
%                   =& \Varmat^H \Varmat \sum_d \sum_{d'} s_ds_{d'}\Kmat{d}^H\Kmat{d} \Kmat{d'}\Kmat{d'}^H
%\matVV[\tnuIndeix,\tnuIndeix']  =& \Exp{(\Varmat\sum_d s_d \Kmat{d})^H(\Varmatprime\sum_d s_d \Kmat{d})} + \mathbf{{I}} \sigma^2\\
%                   =& \Exp{\Varmat^H\Varmatprime}\sum_{d,d'}s_ds_{d'}\Kmat{d}^H\Kmat{d'} + \mathbf{{I}} \sigma^2\\
%\Exp{\Varmat^2}    =& (\matVV - \mathbf{{I}} \sigma^2)\hadam (\sum_{d,d'}s_ds_{d'}\Kmat{d}^H\Kmat{d'})^{\hadam-1} 
\end{align}
%where $\Kmat{d}$ commutes with all other matrices, as it is diagonal.



\subsection{Baseline-based Estimation}

\pg
During calibration, it is customary to assume that there are cells in time and frequency over which the underlying gains are approximately constant. If these cells are known, we then have $N_{\nu}\times N_{t}$ samples to estimate each cell of the covariance matrix, for each baseline. Unfortunately, this is usually not a large number. How to determine the optimal calibration cell size remains an open question, but typical values for LOFAR survey data are of the order of 1 calibration solution every $\sim8$ seconds, and every 4 channels. This means that each weight has about 32 samples, at best, for each estimation: we are far from the 2000 realisations used in our simulations.

\pg
Furthermore, calculating weights for each baseline is quite computationally intensive. In the extreme case, when optimising for fidelity, we invert a $N_t\times N_t$ matrix for each baseline. In practice, this matrix can be approximated as a series of smaller blocks centred around each time, for each baseline: this decreases the cost of inversion, and is equivalent to assuming that the near-diagonal elements of the covariance matrix dominate. Optimising for sensitivity is a lighter task, as only the diagonal elements need be considered: the matrix inversion becomes a set of scalar divisions rather than matrix inversions.

\pg
In spite of these problems, it is possible to use a baseline-based weighting scheme. It is doubtlessly the easiest way to obtain fidelity-optimal weights, and was the method used to obtain Fig. \ref{image.3c295.fullcorr}.


\subsection{Antenna-based Estimation}

\pg
In estimating the covariance matrix for each baseline and each calibration cell, we are severely limited by the small number of samples in each cell. One way to overcome this problem is to find estimates for the variance of \emph{antenna} gains, and use these to return to the baseline variances. Let us begin by writing an expression for the gain vector, which contains the gains for all antennas and all calibration cells:
\begin{align}
\ghatvect_c =& \begin{pmatrix} \vdots \\ \hat{g}_p^{\tnuIndeix\in c} \\ \vdots \end{pmatrix}\\
\ghatvect =& \begin{pmatrix} \hdots \quad \ghatvect_c \quad \hdots \end{pmatrix}
\end{align}
The variance on each antenna in each calibration cell is then:
\begin{align}
\Var{\ghatvect_c} =& \Exp{(\ghatvect_c - \Exp{\ghatvect_c})^H (\ghatvect_c - \Exp{\ghatvect_c}) }\\
               =& \Exp{\ghatvect_c^H \ghatvect_c} - \Exp{\ghatvect_c}^H \Exp{\ghatvect_c}\label{eq.def.vector.variance}
\end{align}
%and we can thus define variance samples as:
%\begin{align}
%\ghatvect
%\end{align}


\pg
As we can see, Eq. \ref{eq.def.vector.variance} is simply a vector form of Eq. \ref{eq.residuals.definition}. Let us therefore extend the hypothesis made in Eq. \ref{eq.gains.independent}.
%This time, however, we must consider the case where $p$ and $q$ are the same antenna:
%\begin{align}
%\Exp{g_{p,\tnuIndeix}g_{q,\tnuIndeix}} =& \Exp{g_{p,\tnuIndeix}}\Exp{g_{q,\tnuIndeix}}\\
%\Exp{g_{p,\tnuIndeix}g_{p,\tnuIndeix}} \ne& \Exp{g_{p,\tnuIndeix}}\Exp{g_{p,\tnuIndeix}}
%\end{align}
%This amounts to assuming that there is \emph{no covariance} between antenna gains, but making no hypotheses on their \emph{variance}. If this holds, then Eq. \ref{eq.def.vector.variance} becomes a diagonal matrix, containing the variance of the estimates for each antenna gain and for one cell in time. 
The residual gains of Eq. \ref{eq.residuals.definition} can now be understood as random samples of the covariance between the gains for antennas $p$ and $q$ at a given time, assuming complete skymodel subtraction. We can thus define the variance sample matrix as an \emph{estimate} of the \emph{variance matrix}:
\begin{align}
\VarmatC =&\widehat{\Var{g_{\tnuIndeix\in\cellindex}}} \\
                   =& \sum_{\tnuIndeix\in\cellindex}\ghatvect_\tnuIndeix^H\ghatvect_\tnuIndeix - \gvect_\tnuIndeix^H\gvect_\tnuIndeix
%\Varmat    =& \gvect^H\gvect - \ghatvect^H\ghatvect
\end{align}
%where the wings of $\VarmatTau$ should average to zero over the gain stability interval, and the diagonal average to the variance of single antennas. % The variance of the antenna gains is then $\ExpVarmat=\Exp{\diag{\Varmat}}$.




\begin{figure*}[t!]
\centering
\begin{subfigure}{.45\textwidth}
\resizebox{\hsize}{!}{\includegraphics{images/3c295-noweights-restored.png}}
%\captionsetup{justification=centering}and I absolutely was like
\caption{\label{image.3c295.nocorr} Uncorrected restored image of the sky near the centre of the Extended Groth Strip. Pixel size is 1.5 arcsec.}
\end{subfigure}
\hfill
\begin{subfigure}{.45\textwidth}
\resizebox{\hsize}{!}{\includegraphics{images/3c295-antweights-restored.png}}
\caption{\label{image.3c295.lightcorr} Sensitivity-optimised restored image of the sky near the centre of the Extended Groth Strip. Pixel size is 1.5 arcsec.}
\end{subfigure}

\begin{subfigure}{.45\textwidth}
\resizebox{\hsize}{!}{\includegraphics{images/3c295-fullweights-restored.png}}
\caption{\label{image.3c295.fullcorr} Artefact-optimised restored image of the sky near the centre of the Extended Groth Strip. Pixel size is 1.5 arcsec.}
\end{subfigure}
\caption{Restored images showing the application of weights}
\end{figure*}


\pg
Note that $\matVV$ then corresponds, quite simply, to the covariance matrix being Fourier transformed over the $\deltu\deltv$ plane in Sec. \ref{sec.formalism}. Sec. \ref{app.sec.matvv} shows what each cell of this matrix corresponds to: each is simply the sum of one of the baseline-dependent quantities calculated in Section \ref{sec.formalism}. We thus average all such quantities within a given time-frequency cell, having now improved our conditioning by a factor of $N_{antenna}$. Finally, we can relate $\matVV$ to the variance of individual antenna gains as follows:
\begin{align}
\matVV[c,c] =& \mathcal{S} \VarmatC\VarmatC + \I\sigma^2\\
\VarmatC    =& \sqrt{\mathcal{S}^{-1}(\matVV[c,c]-\I\sigma^2)}
\end{align}
In other words, $\matVV$ allows us to estimate the variance of each antenna and for each calibration cell. With this information, we can then rebuild the baseline-dependent matrix. The main difference is now that we have improved our sampling by a factor of $N_{ant}$, and open up avenues for computational acceleration. The drawback to this approach is that building the full time-covariance matrix for each baseline becomes once again quite computationally intensive. As such, this approach allows us to better-condition the sensitivity-optimal weight, but was not used to find the artefact-optimal weights.


\section{Applying the Correction to Real Data}



\pg
We now show the effect of our correction algorithm on real data. The dataset used in this section is a single subband from an 8-hour LOFAR observation centred on the Extended Groth Strip. The data have been averaged to 1 data point per 6 seconds, with 8 channels in the subband. The data was calibrated using Wirtinger calibration \citep[see][and references therein]{2014arXiv1410.8706T,2015MNRAS.449.2668S}, solving for one calibration solution per 30 seconds and per 4 channels. This gives us deliberately poor calibration solutions, allowing us to work in a framework where our residual visiblities are dominated by \emph{calibration error}, rather than \emph{sky model incompleteness}.

\pg
The pixel size in all of these images is 1.5 arcsec/pixel. Briggs weighting was applied automatically. All the images were made using the same data with same imaging parameters - the only difference is the application of different versions of the weighting scheme proposed in this paper.
Fig. \ref{image.3c295.nocorr} shows an image made without applying any weighting scheme. This is a restored image; deconvolution has been performed.
Applying the sensitivity-optimal weighting scheme described in Sec. \ref{section.algorithm}, we find the image shown in Fig. \ref{image.3c295.lightcorr}. Note that many of the artefacts in the field have decreased, and that fainter sources appear. These weights do not take time-covariance into account, and were calculated in 1min6s on a single core.
Applying the artefact-optimal weighting scheme described in Sec. \ref{section.algorithm}, we find the image shown in Fig. \ref{image.3c295.fullcorr}. Note that we now see many of the fainter sources which were previously well below noise level. The weights here take into account the time-covariance of each antenna's residual visibilities with the 250 nearest time cells. This number was chosen since it corresponds to the 50 neighbouring calibration solution intervals. The weights were calculated in 1h25min. The computational cost associated with calculating the \emph{full} covariance-dependent weights is thus non-negligible. % - but since we are calculating per-antenna weights, the problem is embarrassingly parallelisable in that each antenna weight can be calculated separately from all others. In this case, we have 62 antennas.


==> source/flattening-simulations.tex <==
\subsection{Applying the Correction to Simulated Data}\label{section.simulations.application}


\begin{figure}[!t]
    \centering
%    \begin{subfigure}{0.45\textwidth}
%        \centering
%        \includegraphics[width=\linewidth]{images/ctime099-NoisePsfCrossections.png} 
%        \caption{The sensitivity-optimal (green) and artefact-optimal (red) weights give improvements over the raw noise-PSF (blue), though the full-correction tail is higher than the others.} \label{plot.ctime000.applycorr}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/ctime001-NoisePsfCrossections-backup.png} 
        \caption{The sensitivity-optimal (green) and artefact-optimal (red) weights both give improvements over the raw noise-PSF (blue).} \label{fig.simu.weightapplied}
%    \end{subfigure}
        % just an empty subfigure to shift C below A
%    \caption{Some general caption of all the figures. In (\subref{fig:timing1}) you can see a  green square....}
%\caption{Weight-corrected noise-PSF}
\end{figure}

\pg
In this section, we show the impact of our weighting schemes on an arbitrary strongly-peaked noise-PSF. The cross-section is taken from $\left(l,m\right)=0$ to a large $l$, keeping $m$ constant. The only difference between these cross-sections is the weighting scheme applied: unit weights for all visibilities (``Uncorrected", blue), sensitivity-optimal weights (green), and artefact-optimal weights (red). We plot both the result predicted by the Cov-Cov relationship (solid line) and the variance estimated across 2000 realisations (dashed line): the result is shown in Fig. \ref{fig.simu.weightapplied}. The two remain in such agreement throughout the cross-section as to be nearly indistinguishable. 

\pg
There are a few significant points to note on this figure. Firstly, most of the power in the matrix lies along the diagonal: both weighting schemes thus give good improvements in variance across the map. The artefact-optimal weights, while decreasing the peak further, as expected, also increases the noise far from sources: this is due to the fact that the artefact-optimal weights are in a sense more ``selective" than the sensitivity-optimal weights: they up-weigh and down-weigh more severely, and will only result in a constant covariance matrix if this matrix is zero everywhere outside of the diagonal. {In effect, the noise-PSF becomes flatter, but much broader.}



%\pg
%The cvariance matrix of our residual visibilities has real values along its diagonal, but its wings consist entirely of complex numbers. As such, the ``true" full-correction weights must, too, be complex. In Fig. \ref{plot.ctime000.applycorr}, the absolute value of the complex weights were used, to remain consistent with common practice. Using complex weights has an impressive advantage, however: it fully flattens the noise-PSF. This is shown in Fig. \ref{plot.ctime000.applycorr.complexweights}.\\
%
%\pg
%This improvement is due to the fact that taking the absolute value of the complex number results in a loss of information, thus deteriorating the improvement of full-correction when using real weights. Since correlated phase residuals are likely to be indicative of a visibility for which phase calibration was poor, this flattening of the noise-PSF should correspond to applying a phase correction proportional to this error for each visibility and each time. This would only hold in the absence of direction-dependent effects, and assuming we have a good estimate of the baseline-dependent covariance matrix.
